Generative AI in Cybersecurity: A Comprehensive Review of LLM Applications and Vulnerabilities

This paper provides a comprehensive review of the future of cybersecurity through Generative AI and Large Language Models (LLMs). We explore LLM applications across various domains, including hardware design security, intrusion detection, software engineering, design verification, cyber threat intelligence, malware detection, and phishing detection. We present an overview of LLM evolution and its current state, focusing on advancements in models such as GPT-4, GPT-3.5, Mixtral-8x7B, BERT, Falcon2, and LLaMA. Our analysis extends to LLM vulnerabilities, such as prompt injection, insecure output handling, data poisoning, DDoS attacks, and adversarial instructions. We delve into mitigation strategies to protect these models, providing a comprehensive look at potential attack scenarios and prevention techniques. Furthermore, we evaluate the performance of 42 LLM models in cybersecurity knowledge and hardware security, highlighting their strengths and weaknesses. We thoroughly evaluate cybersecurity datasets for LLM training and testing, covering the lifecycle from data creation to usage and identifying gaps for future research. In addition, we review new strategies for leveraging LLMs, including techniques like Half-Quadratic Quantization (HQQ), Reinforcement Learning with Human Feedback (RLHF), Direct Preference Optimization (DPO), Quantized Low-Rank Adapters (QLoRA), and Retrieval-Augmented Generation (RAG). These insights aim to enhance real-time cybersecurity defenses and improve the sophistication of LLM applications in threat detection and response. Our paper provides a foundational understanding and strategic direction for integrating LLMs into future cybersecurity frameworks, emphasizing innovation and robust model deployment to safeguard against evolving cyber threats.

==> HWtable.tex <==
\begin{table*}[]
\centering
\caption{Comparison of 19 LLMs Models' Performance in hardware security Knowledge.}
\label{tab:llmhwsec}
\begin{tabular}{|c|c|c|c|ccccccccc|}
\hline
\multirow{2}{*}{\textbf{LLM model}} & \multirow{2}{*}{\textbf{Size}} & \multicolumn{9}{c|}{\textbf{Hardware CWE}}                                                                                                                                                                                             \\ \cline{5-13} 
                                    &                                   &                                &                                   & \multicolumn{1}{c|}{\textbf{cwe 1245 }} & \multicolumn{1}{c|}{\textbf{cwe 1221}} & \multicolumn{1}{c|}{\textbf{cwe 1224}} & \multicolumn{1}{c|}{\textbf{cwe 1298}}
                                    & \multicolumn{1}{c|}{\textbf{cwe 1245}} & \multicolumn{1}{c|}{\textbf{cwe 1209}} & \multicolumn{1}{c|}{\textbf{cwe 1223}} & \multicolumn{1}{c|}{\textbf{cwe 1234}}
                                    & \textbf{cwe 1231}
                                    
                                    \\ \hline
\cellcolor{green!100} mistral-openorca & N/A & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}   & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{96.25\%} & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{N/A} & N/A\%  \\ \hline

\cellcolor{green!100} dolphin-mistral & N/A & N/A & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}   & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A\%} & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{N/A} & N/A\%  \\ \hline

\cellcolor{green!100} codegemma & N/A & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}   & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{N/A} & N/A\%  \\ \hline

\cellcolor{green!100} orca-mini & N/A & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}   & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A}  & \multicolumn{1}{c|}{N/A} & N/A\%  \\ \hline

\end{tabular}
\end{table*}

==> future.tex <==
\section{Opportunities and Future Directions}
\label{sec:future}


\subsection{Building an instruction Cyber Security dataset}
\subsection{Pre-training models}
\subsection{Supervised Fine-Tuning}
\subsection{Reinforcement Learning from Human Feedback}
\subsection{Quantization}
\subsection{Inference optimization}

==> sections/background.tex <==
\section{Background for LLMs in Software Testing}
\label{sec:background}


\subsection{Cyber Security}
Cyber security is a comprehensive term that protects all aspects of digital systems, networks, and data from a wide range of cyber threats. Cyber security extends beyond individual software applications to encompass the entire technology infrastructure, including hardware, software, networks, devices, and the people who use and manage them. 
Cyber security safeguards digital systems and sensitive data from malicious threats. 



